Matrix Completion in Almost-Verification Time

We give a new framework for solving the fundamental problem of low-rank matrix completion, i.e., approximating a rank-$r$ matrix $\mathbf{M} \in \mathbb{R}^{m \times n}$ (where $m \ge n$) from random observations. First, we provide an algorithm which completes $\mathbf{M}$ on $99\%$ of rows and columns under no further assumptions on $\mathbf{M}$ from $\approx mr$ samples and using $\approx mr^2$ time. Then, assuming the row and column spans of $\mathbf{M}$ satisfy additional regularity properties, we show how to boost this partial completion guarantee to a full matrix completion algorithm by aggregating solutions to regression problems involving the observations. In the well-studied setting where $\mathbf{M}$ has incoherent row and column spans, our algorithms complete $\mathbf{M}$ to high precision from $mr^{2+o(1)}$ observations in $mr^{3 + o(1)}$ time (omitting logarithmic factors in problem parameters), improving upon the prior state-of-the-art [JN15] which used $\approx mr^5$ samples and $\approx mr^7$ time. Under an assumption on the row and column spans of $\mathbf{M}$ we introduce (which is satisfied by random subspaces with high probability), our sample complexity improves to an almost information-theoretically optimal $mr^{1 + o(1)}$, and our runtime improves to $mr^{2 + o(1)}$. Our runtimes have the appealing property of matching the best known runtime to verify that a rank-$r$ decomposition $\mathbf{U}\mathbf{V}^\top$ agrees with the sampled observations. We also provide robust variants of our algorithms that, given random observations from $\mathbf{M} + \mathbf{N}$ with $\|\mathbf{N}\|_{F} \le \Delta$, complete $\mathbf{M}$ to Frobenius norm distance $\approx r^{1.5}\Delta$ in the same runtimes as the noiseless setting. Prior noisy matrix completion algorithms [CP10] only guaranteed a distance of $\approx \sqrt{n}\Delta$.

==> noise-verification.tex <==
\section{Noise level verification}


In this section, we show that our algorithm can be made agnostic to the noise level $\normf{N}$.  To do this, it suffices to estimate the error between the true matrix and the matrix returned by our algorithm using random observations.  Recall that the matrix we output has an $(\alpha , \beta)$-regular column space and the true matrix has $(\alpha , \beta)$-regular row and column spaces.  Thus to show that we can estimate the error, it suffices to prove the following generic statement about the difference between two such matrices being witnessed by random entries with high probability.

\begin{lemma}\label{lem:diff-between-regular}
Let $\mm, \mm' \in \R^{m \times n}$ be matrices with rank at most $r$.  Assume that $\mm$ has $(\alpha , \beta)$-regular row and column spaces and $\mm'$ has an $(\alpha , \beta)$-regular column space.  Let $S \subset [m] \times [n]$ be drawn by including each element independently with probability $p \geq \frac{10^{12}r}{\alpha \beta^6 \min(m,n)}\log(mn)$.  Then with probability $0.99$,
\[
\sum_{(i,j) \in S}(\mm_{ij} - \mm_{ij}')^2 \geq   (0.1\beta)^4 p   \normf{\mm - \mm'}^2
\]
\end{lemma}


To prove Lemma~\ref{lem:diff-between-regular}, we break into two cases.  We first consider the case where the difference $\mm - \mm'$ is somewhat spread out over all of the columns.


\begin{claim}\label{claim:case-1}
Let $\mm, \mm' \in \R^{m \times n}$ be matrices with rank at most $r$.  Assume that $\mm$ has $(\alpha , \beta)$-regular row and column spaces and $\mm'$ has an $(\alpha , \beta)$-regular row space.  Let $\Delta = \normf{\mm - \mm'}$.  Let $T \subset [n]$ consist of the indices $j$ such that $\norm{\mm_{:j} - \mm'_{:j}} \leq \Delta \sqrt{p}\beta^2/10^3$.  Assume that
\[
\normf{\mm_{:T} - \mm'_{:T}}^2 \geq 2 \cdot (0.1\beta)^4 \Delta^2 \,.
\]
Let $S \subset [m] \times [n]$ be drawn by including each element independently with probability $p$.  Then with probability $0.9$,
\[
\sum_{(i,j) \in S}(\mm_{ij} - \mm_{ij}')^2 \geq   p (0.1 \beta)^4 \Delta^2
\]  
\end{claim}
\begin{proof}
Let $D = \mm - \mm'$.  Define the random variable $X = \sum_{(i,j) \in S, j \in T}D_{ij}^2$ where the randomness is in the selection of $S$.  We have 
\[
\E[X'] = p\normf{\mm_{:T} - \mm'_{:T}}^2  \,. 
\]
We also have
\[
\begin{split}
\E[X'^2] - \E[X']^2 \leq p\sum_{(i,j) \in S, j \in T} D_{ij}^4 \leq  p\sum_{j \in T}\norm{\mm_{:j} - \mm'_{:j}}^4 \leq p\normf{\mm_{:T} - \mm'_{:T}}^2 \cdot  \frac{\Delta^2 \beta^4 p}{10^6} \\ \leq \frac{1}{200} \E[X']^2 \,.
\end{split}
\]
Thus with $0.95$ probability, $X \geq 0.5\E[X'] \geq p(0.1 \beta)^4 \Delta^2$ and clearly $\sum_{(i,j) \in S}(\mm_{ij} - \mm_{ij}')^2 \geq X$ so we are done.
\end{proof}


Next, we consider the case when the difference $\mm - \mm'$ is concentrated on a very small number of columns.  Roughly, we will prove that $\mm'$ is actually very close (much closer than $\normf{\mm - \mm'}$) to a matrix with the same column-span as $\mm$ so most of the difference actually lives in an $(\alpha, \beta)$-regular column space.  Then we will invoke the following basic observation. 

\begin{claim}\label{claim:estimate-regular-column-space}
Let $\mn \in \R^{m \times n}$ be a rank-$r$ matrix with an $(\alpha, \beta)$-regular column space.  Let $p \in [0,1]$ be some parameter with $p \geq \frac{10^{12}r}{\alpha \beta^2 \min(m,n)}\log(mn)$.  Let $S \subset [m] \times [n]$ be a random subset where each element is included independently with probability $p$.  Then with probability $0.99$,
\[
\sum_{(i,j) \in S} \mn_{ij}^2 \geq \frac{p\beta^2}{2} \normf{\mn}^2 \,.
\]
\end{claim}
\begin{proof}
Let $\mmu$ be an orthonormal basis for the column space of $\mn$.  Now we apply Lemma~\ref{lem:regular-lower-bound}  on each column with $\delta = 1/(100n)$.  For each $j \in [n]$, let $S_j$ be the set of $i$ such that $(i,j) \in S$.  If the conclusion of Lemma~\ref{lem:regular-lower-bound} holds for a given value of $j$ then
\[
\sum_{i \in S_j} \mn_{ij}^2 \geq \frac{p\beta^2}{2} \norm{\mn_{:j}}^2 \,.
\]
Union bounding and summing over all $j \in [n]$ gives the desired inequality.  
\end{proof}


\begin{claim}\label{claim:case-2}
Let $\mm, \mm' \in \R^{m \times n}$ be matrices with rank at most $r$.  Assume that $\mm$ has $(\alpha , \beta)$-regular row and column spaces and $\mm'$ has an $(\alpha , \beta)$-regular row space.  Let $\Delta = \normf{\mm - \mm'}$.  Let $p \in [0,1]$ be some parameter with $p \geq \frac{10^{12}r}{\alpha \beta^6 \min(m,n)}\log(mn)$.  Let $T \subset [n]$ consist of the indices $j$ such that $\norm{\mm_{:j} - \mm'_{:j}} \leq \Delta \sqrt{p}\beta^2 /10^3$.  Assume that
\[
\normf{\mm_{:T} - \mm'_{:T}}^2 \leq 2 \cdot (0.1 \beta)^4 \Delta^2 \,.
\]
Let $S \subset [m] \times [n]$ be drawn by including each element independently with probability $p$.  Then with probability $0.7$,
\[
\sum_{(i,j) \in S}(\mm_{ij} - \mm_{ij}')^2 \geq   p (0.1\beta)^4 \Delta^2
\]  
\end{claim}

\begin{proof}
Let $Q \subset [n]$ be drawn by including each element with probability $p' = \beta^4 p/10^8$.  Let $\mv \in \R^{r \times n}$ have rows forming an orthonormal basis of $\mm$ and $\mv' \in \R^{r \times n}$ have rows forming an orthonormal basis of $\mm'$.  By Lemma~\ref{lem:regular-lower-bound} and Fact~\ref{fact:mu_alpha}, with probability $0.99$, we have
\[
\begin{split}
\sum_{j \in Q} \mv_{:j}(\mv_{:j})^\top \succeq \frac{p'\beta^2}{2} \id_r & \\
\sum_{j \in Q} \mv_{:j}'(\mv_{:j}')^\top \succeq \frac{p'\beta^2}{2} \id_r \,.
\end{split}
\]
This implies that there are matrices $\mn, \mn' \in \R^{|Q| \times n}$ with $\normop{\mn}, \normop{\mn'} \leq \frac{\sqrt{2}}{\sqrt{p'}\beta}$ such that $\mv_{:Q}\mn = \mv$ and $\mv'_{:Q}\mn' = \mv'$.  Now recall that we can write $\mm = \mmu \mv, \mm' = \mmu' \mv'$ for some matrices $\mmu, \mmu'$.  Note that by Markov's inequality $|[n] \backslash T| \leq 10^6/(\beta^4 p) \leq \frac{1}{100 p'}$.  Thus with probability $0.99$, $Q \subset T$.  Applying Markov's inequality again, we conclude that with $0.8$ probability, 
\[
\normf{\mm_{:Q} - \mm'_{:Q}}^2 \leq 5 p' \normf{\mm_{:T} - \mm'_{:T}}^2 \leq \frac{p'\beta^4 \Delta^2}{10^3} \,.
\]
In particular, such a set $Q$ satisfying all of the above conditions exists.  From now on we can fix this set $Q$.  The randomness we consider from now on is only in the elements of $S$.  The above implies that 
\[
\normf{\mm_{:Q}\mn' - \mm'} = \normf{\mm_{:Q}\mn' - \mm'_{:Q}\mn'} \leq \frac{ \beta \Delta}{20} \,.
\]
Now define the matrices $F = \mm - \mm_{:Q}\mn'$ and $G = \mm_{:Q}\mn' - \mm'$.  Note that the column space of $D_1$ is $(\alpha , \beta)$-regular.  Thus, with probability $0.99$ over the randomness of $S$
\[
d_F = \sum_{(i,j) \in S} F_{ij}^2  \geq \frac{p \beta^2}{2} \normf{F}^2 \geq 0.4p\beta^2 \Delta^2
\]
where in the last step we used the triangle inequality to derive $\normf{F} \geq \Delta - \normf{G} \geq (1 - \beta/20)\Delta$.  Also, by Markov's inequality, with probability $0.95$,
\[
d_G = \sum_{(i,j) \in S} G_{ij}^2 \leq 20 p \normf{G}^2 \leq \frac{p\beta^2 \Delta^2}{20} \,.
\]
Combining the above and using the triangle inequality, we conclude that with probability $0.9$ over the randomness of $S$, 
\[
\sum_{(i,j) \in S}(\mm_{ij} - \mm_{ij}')^2 \geq \left(\sqrt{d_F} - \sqrt{d_G}  \right)^2 \geq 0.1 p\beta^2\Delta^2 
\]
\end{proof}


\begin{proof}[Proof of Lemma~\ref{lem:diff-between-regular}]
It follows trivially from combining Claim~\ref{claim:case-1} and Claim~\ref{claim:case-2}.
\end{proof}



Now we can obtain the following corollary that generalizes our main theorem to the case when the noise level $\normf{N}$ is unknown.  We can simply start with $\Delta$ set to an upper bound on $\normf{N}$ and repeatedly apply Theorem~\ref{thm:main} and check the error of our output and then decrease $\Delta$ by a factor of $2$.  

\begin{corollary}\label{coro:main-thm-unknown-error}
Let $\mms \in \R^{m \times n}$ be rank-$\rs$ with $(\alpha, \mu, \beta)$-standard row and column spans, $m \ge n$, $\delta \in (0, 1)$, and let $\mmh = \mms + \mn$ for some unknown noise matrix $\mn$.  Assume we are given some lower bound $\Delta_{\min}$ on the desired accuracy.  There is an algorithm that returns $\mmu \in \R^{m \times r}$ and $\mv \in \R^{n \times r}$ for $r \le 2\rs$, satisfying
$\normf{\mmu \mv^\top - \mms} \le \frac{(\rs)^{1.5 + o(1)}}{\beta^{11}} \normf{\mn}$,
with probability $\ge 1 - \delta$ and using
\[O\Par{\frac{m(\rs)^{2 + o(1)} \mu^2}{\alpha \beta^{6 + o(1)}} \cdot \Par{\log^6\Par{\frac m {\alpha\beta\delta}}\log\Par{\frac{m\normop{\mms}}{\normf{\mn}\beta\delta}} + \log^{2.5}\Par{\frac m {\alpha\beta\delta}}\log^2\Par{\frac{m\normop{\mms}}{\normf{\mn}\beta\delta}} } }\]
time and one call to $\oracle_p(\mmh)$ where for a sufficiently large constant,
\[p = O\Par{\frac{(\rs)^{1 + o(1)} \mu }{\alpha \beta^{2 + o(1)} n} \cdot \log^{6}\Par{\frac m {\alpha\beta\delta}}\log\Par{\frac{n\normop{\mms}}{\normf{\mn}}}}.\]
\end{corollary}
\begin{proof}
\allen{Add note to Theorem~\ref{thm:main} that one of the subspaces is regular} Apply Lemma~\ref{lem:approx_op_norm} to obtain an upper bound $\Delta_0$ on $\normf{\mms}$ which we can also use as an upper bound on $\normf{N}$.  Now we will iteratively apply Theorem~\ref{thm:main}, check the error of our output, and decrease $\Delta_{i+1} = \Delta_i/2$.  Let $\mm' = \mmu \mv^\top$ be the output. It is clear from the proof of Theorem~\ref{thm:main} that the output has an $(\alpha , \beta/2)$-regular column space.  Now let 
\[
p' = \frac{Cr}{\alpha \beta^6 n}\log(mn)
\]
for some sufficiently large constant $C$.  Now draw  $l = 10\log(mn/\delta)$ random sets $S_1, \dots , S_l \subset [m] \times [n]$ where each element is included with probability $p'$.  For each, compute the quantity
\[
d_l = \frac{\sqrt{\sum_{(i,j) \in S}(\mmh_{ij} - \mm_{ij}')^2 } }{\sqrt{p'}}
\]
and let $d_{\textsf{est}}$ be the median.  By Lemma~\ref{lem:diff-between-regular}and Markov's inequality, we have
with $1 - (\delta/mn)^2$ probability,
\[
0.01\beta^2 \normf{\mms - \mm'} - 10\normf{\mn}  \leq d_{\textsf{est}} \leq 10(\normf{\mms - \mm'} + \normf{\mn}) \,.
\]
\end{proof}

